Parallelism in Randomized Incremental Algorithms

In this paper we show that many sequential randomized incremental algorithms are in fact parallel. We consider algorithms for several problems including Delaunay triangulation, linear programming, closest pair, smallest enclosing disk, least-element lists, and strongly connected components. We analyze the dependences between iterations in an algorithm, and show that the dependence structure is shallow with high probability, or that by violating some dependences the structure is shallow and the work is not increased significantly. We identify three types of algorithms based on their dependences and present a framework for analyzing each type. Using the framework gives work-efficient polylogarithmic-depth parallel algorithms for most of the problems that we study. This paper shows the first incremental Delaunay triangulation algorithm with optimal work and polylogarithmic depth, which is an open problem for over 30 years. This result is important since most implementations of parallel Delaunay triangulation use the incremental approach. Our results also improve bounds on strongly connected components and least-elements lists, and significantly simplify parallel algorithms for several problems.

==> bbl.tex <==
\begin{thebibliography}{10}

\bibitem{Ajtai1992}
M.~Ajtai and N.~Megiddo.
\newblock A deterministic poly$(\log \log n)$-time $n$-processor algorithm for
  linear programming in fixed dimension.
\newblock In {\em ACM Symposium on Theory of Computing (STOC)}, pages 327--338,
  1992.

\bibitem{Alon1994}
N.~Alon and N.~Megiddo.
\newblock Parallel linear programming in fixed dimension almost surely in
  constant time.
\newblock {\em J. ACM (JACM)}, 41(2):422--434, Mar. 1994.

\bibitem{AG93}
M.~Atallah and M.~Goodrich.
\newblock Deterministic parallel computational geometry.
\newblock In {\em Synthesis of Parallel Algorithms}, pages 497--536. Morgan
  Kaufmann, 1993.

\bibitem{barnat2011computing}
J.~Barnat, P.~Bauch, L.~Brim, and M.~Ceska.
\newblock Computing strongly connected components in parallel on {CUDA}.
\newblock In {\em International Parallel \& Distributed Processing Symposium
  (IPDPS)}, pages 544--555, 2011.

\bibitem{BBK06}
D.~K. Blandford, G.~E. Blelloch, and C.~Kadow.
\newblock Engineering a compact parallel {Delaunay} algorithm in {3D}.
\newblock In {\em {ACM} Symposium on Computational Geometry (SoCG)}, pages
  292--300, 2006.

\bibitem{BFGS}
G.~E. Blelloch, J.~T. Fineman, P.~B. Gibbons, and J.~Shun.
\newblock Internally deterministic algorithms can be fast.
\newblock In {\em Principles and Practice of Parallel Programming (PPoPP)},
  pages 181--192, 2012.

\bibitem{BFS12}
G.~E. Blelloch, J.~T. Fineman, and J.~Shun.
\newblock Greedy sequential maximal independent set and matching are parallel
  on average.
\newblock In {\em ACM Symposium on Parallelism in Algorithms and Architectures
  (SPAA)}, pages 308--317, 2012.

\bibitem{FRTnew}
G.~E. Blelloch, Y.~Gu, and Y.~Sun.
\newblock Efficient construction of probabilistic tree embeddings.
\newblock {\em arXiv preprint: 1605.04651}, 2016.

\bibitem{Blelloch16shortest}
G.~E. Blelloch, Y.~Gu, Y.~Sun, and K.~Tangwongsan.
\newblock Parallel shortest-paths using radius stepping.
\newblock In {\em ACM Symposium on Parallelism in Algorithms and Architectures
  (SPAA)}, 2016.

\bibitem{kanat}
G.~E. Blelloch, A.~Gupta, and K.~Tangwongsan.
\newblock Parallel probabilistic tree embeddings, k-median, and buy-at-bulk
  network design.
\newblock In {\em ACM Symposium on Parallelism in Algorithms and
  Architectures (SPAA)}, pages 205--213, 2012.

\bibitem{BHMT99}
G.~E. Blelloch, J.~C. Hardwick, G.~L. Miller, and D.~Talmor.
\newblock Design and implementation of a practical parallel {Delaunay}
  algorithm.
\newblock {\em Algorithmica}, 24(3-4):243--269, 1999.

\bibitem{Bocchino09}
R.~L. Bocchino, V.~S. Adve, S.~V. Adve, and M.~Snir.
\newblock Parallel programming must be deterministic by default.
\newblock In {\em Usenix HotPar}, 2009.

\bibitem{BT93}
J.-D. Boissonnat and M.~Teillaud.
\newblock On the randomized construction of the delaunay tree.
\newblock {\em Theoretical Computer Science}, 112(2):339--354, 1993.

\bibitem{brent1974parallel}
R.~P. Brent.
\newblock The parallel evaluation of general arithmetic expressions.
\newblock {\em J. ACM (JACM)}, 21(2):201--206, 1974.

\bibitem{Stamp08}
C.~Cao~Minh, J.~Chung, C.~Kozyrakis, and K.~Olukotun.
\newblock {STAMP}: Stanford transactional applications for multi-processing.
\newblock In {\em IEEE International Symposium on Workload Characterization
  (IISWC)}, 2008.

\bibitem{Chen2002}
D.~Z. Chen and J.~Xu.
\newblock Two-variable linear programming in parallel.
\newblock {\em Computational Geometry}, 21(3):155 -- 165, 2002.

\bibitem{Cignoni}
P.~Cignoni, C.~Montani, R.~Perego, and R.~Scopigno.
\newblock Parallel 3D delaunay triangulation.
\newblock {\em Computer Graphics Forum}, 12(3):129--142, 1993.

\bibitem{Cintra2004}
M.~Cintra, D.~R. Llanos, and B.~Palop.
\newblock International conference on computational science and its
  applications.
\newblock In {\em Speculative Parallelization of a Randomized Incremental
  Convex Hull Algorithm}, pages 188--197, 2004.

\bibitem{CS89}
K.~L. Clarkson and P.~W. Shor.
\newblock Applications of random sampling in computational geometry, {II}.
\newblock {\em Discrete \& Computational Geometry}, 4(5):387--421, 1989.

\bibitem{cohen1997}
E.~Cohen.
\newblock Size-estimation framework with applications to transitive closure and
  reachability.
\newblock {\em Journal of Computer and System Sciences}, 55(3):441--453, 1997.

\bibitem{cohen2004}
E.~Cohen and H.~Kaplan.
\newblock Efficient estimation algorithms for neighborhood variance and other
  moments.
\newblock In {\em ACM-SIAM Symposium on Discrete Algorithms (SODA)}, pages
  157--166, 2004.

\bibitem{Cole88}
R.~Cole.
\newblock Parallel merge sort.
\newblock {\em SIAM J. Comput.}, 17(4):770--785, 1988.

\bibitem{coppersmith2003}
D.~Coppersmith, L.~Fleischer, B.~Hendrickson, and A.~Pinar.
\newblock A divide-and-conquer algorithm for identifying strongly connected
  components.
\newblock Technical Report RC23744, IBM, 2003.

\bibitem{BCKO}
M.~de~Berg, O.~Cheong, M.~van Kreveld, and M.~Overmars.
\newblock {\em Computational Geometry: Algorithms and Applications}.
\newblock Springer-Verlag, 2008.

\bibitem{Deng1990}
X.~Deng.
\newblock An optimal parallel algorithm for linear programming in the plane.
\newblock {\em Information Processing Letters}, 35(4):213 -- 217, 1990.

\bibitem{Diaz04}
P.~Diaz, D.~R. Llanos, and B.~Palop.
\newblock Parallelizing {2D}-convex hulls on clusters: Sorting matters.
\newblock {\em Jornadas De Paralelismo}, 2004.

\bibitem{du2013}
N.~Du, L.~Song, M.~Gomez-Rodriguez, and H.~Zha.
\newblock Scalable influence estimation in continuous-time diffusion networks.
\newblock In {\em Advances in Neural Information Processing Systems (NIPS)},
  pages 3147--3155, 2013.

\bibitem{Dyer1995}
M.~Dyer.
\newblock A parallel algorithm for linear programming in fixed dimension.
\newblock In {\em Symposium on Computational Geometry (SoCG)}, pages 345--349,
  1995.

\bibitem{Edelsbrunner06}
H.~Edelsbrunner.
\newblock {\em Geometry and Topology for Mesh Generation}.
\newblock Cambridge University Press, 2006.

\bibitem{FRT}
J.~Fakcharoenphol, S.~Rao, and K.~Talwar.
\newblock A tight bound on approximating arbitrary metrics by tree metrics.
\newblock {\em Journal of Computer and System Sciences (JCSS)}, 69(3):485--497,
  2004.

\bibitem{Gil91a}
J.~Gil, Y.~Matias, and U.~Vishkin.
\newblock Towards a theory of nearly constant time parallel algorithms.
\newblock In {\em Foundations of Computer Science (FOCS)}, pages 698--710,
  1991.

\bibitem{Golin1995}
M.~Golin, R.~Raman, C.~Schwarz, and M.~Smid.
\newblock Simple randomized algorithms for closest pair problems.
\newblock {\em Nordic J. of Computing}, 2(1):3--27, Mar. 1995.

\bibitem{Gonzalez2006}
A.~Gonzalez-Escribano, D.~R. Llanos, D.~Orden, and B.~Palop.
\newblock Parallelization alternatives and their performance for the convex
  hull problem.
\newblock {\em Applied Mathematical Modelling}, 30(7):563 -- 577, 2006.

\bibitem{Goodrich1996}
M.~T. Goodrich.
\newblock Fixed-dimensional parallel linear programming via relative
  $\epsilon$-approximations.
\newblock In {\em ACM-SIAM Symposium on Discrete Algorithms (SODA)}, pages
  132--141, 1996.

\bibitem{Goodrich97}
M.~T. Goodrich and E.~A. Ramos.
\newblock Bounded-independence derandomization of geometric partitioning with
  applications to parallel fixed-dimensional linear programming.
\newblock {\em Discrete \& Computational Geometry}, 18(4):397--420, 1997.

\bibitem{GrSi78}
P.~J. Green and R.~Sibson.
\newblock Computing {Dirichlet} tessellations in the plane.
\newblock {\em The Computer Journal}, 21(2):168--173, 1978.

\bibitem{GSSB15}
Y.~Gu, J.~Shun, Y.~Sun, and G.~E. Blelloch.
\newblock A top-down parallel semisort.
\newblock In {\em ACM Symposium on Parallelism in Algorithms and Architectures
  (SPAA)}, pages 24--34, 2015.

\bibitem{GKS92}
L.~J. Guibas, D.~E. Knuth, and M.~Sharir.
\newblock Randomized incremental construction of {Delaunay} and {Voronoi}
  diagrams.
\newblock {\em Algorithmica}, 7(4):381--413, 1992.

\bibitem{Har-peled2011}
S.~Har-peled.
\newblock {\em Geometric Approximation Algorithms}.
\newblock American Mathematical Society, 2011.

\bibitem{hasenplaugh2014ordering}
W.~Hasenplaugh, T.~Kaler, T.~B. Schardl, and C.~E. Leiserson.
\newblock Ordering heuristics for parallel graph coloring.
\newblock In {\em ACM Symposium on Parallelism in Algorithms and Architectures
  (SPAA)}, pages 166--177, 2014.

\bibitem{hong2013fast}
S.~Hong, N.~C. Rodia, and K.~Olukotun.
\newblock On fast parallel detection of strongly connected components ({SCC})
  in small-world graphs.
\newblock In {\em International Conference for High Performance Computing,
  Networking, Storage and Analysis (SC)}, pages 1--11, 2013.

\bibitem{JaJa92}
J.~Jaja.
\newblock {\em Introduction to Parallel Algorithms}.
\newblock Addison-Wesley Professional, 1992.

\bibitem{khan2012}
M.~Khan, F.~Kuhn, D.~Malkhi, G.~Pandurangan, and K.~Talwar.
\newblock Efficient distributed approximation algorithms via probabilistic tree
  embeddings.
\newblock {\em Distributed Computing}, 25(3):189--205, 2012.

\bibitem{Khuller1995}
S.~Khuller and Y.~Matias.
\newblock A simple randomized sieve algorithm for the closest-pair problem.
\newblock {\em Information and Computation}, 118(1):34--37, 1995.

\bibitem{klein1997randomized}
P.~N. Klein and S.~Subramanian.
\newblock A randomized parallel algorithm for single-source shortest paths.
\newblock {\em Journal of Algorithms}, 25(2):205--220, 1997.

\bibitem{Llanos05}
D.~R. Llanos, D.~Orden, and B.~Palop.
\newblock Meseta: A new scheduling strategy for speculative parallelization of
  randomized incremental algorithms.
\newblock {\em International Conference on Parallel Processing Workshops},
  pages 121--128, 2005.

\bibitem{Megiddo83}
N.~Megiddo.
\newblock Linear-time algorithms for linear programming in {$R^3$} and related
  problems.
\newblock {\em SIAM Journal on Computing}, 1983.

\bibitem{Mulmuley94}
K.~Mulmuley.
\newblock {\em Computational geometry - an introduction through randomized
  algorithms}.
\newblock Prentice Hall, 1994.

\bibitem{PanPORRJ15}
X.~Pan, D.~Papailiopoulos, S.~Oymak, B.~Recht, K.~Ramchandran, and M.~I.
  Jordan.
\newblock Parallel correlation clustering on big graphs.
\newblock In {\em Advances in Neural Information Processing Systems (NIPS)},
  2015.

\bibitem{Pingali11}
K.~Pingali, D.~Nguyen, M.~Kulkarni, M.~Burtscher, M.~A. Hassaan, R.~Kaleem,
  T.-H. Lee, A.~Lenharth, R.~Manevich, M.~M\'{e}ndez-Lojo, D.~Prountzos, and
  X.~Sui.
\newblock The tao of parallelism in algorithms.
\newblock In {\em ACM SIGPLAN conference on Programming Language Design and
  Implementation (PLDI)}, 2011.

\bibitem{Rabin76}
M.~O. Rabin.
\newblock Probabilistic algorithms.
\newblock {\em Algorithms and Complexity: New Directions and Recent Results},
  pages 21--39, 1976.

\bibitem{RR89}
S.~Rajasekaran and J.~H. Reif.
\newblock Optimal and sublogarithmic time randomized parallel sorting
  algorithms.
\newblock {\em SIAM J. Comput.}, 18(3):594--607, 1989.

\bibitem{reif1985}
J.~H. Reif.
\newblock Depth-first search is inherently sequential.
\newblock {\em Information Processing Letters}, 20(5):229--234, 1985.

\bibitem{RS92}
J.~H. Reif and S.~Sen.
\newblock Optimal randomized parallel algorithms for computational geometry.
\newblock {\em Algorithmica}, 7(1-6):91--117, 1992.

\bibitem{schudy2008finding}
W.~Schudy.
\newblock Finding strongly connected components in parallel using {$O(\log^2
  n)$} reachability queries.
\newblock In {\em ACM Symposium on Parallelism in Algorithms and Architectures
  (SPAA)}, pages 146--151, 2008.

\bibitem{Seidel1991}
R.~Seidel.
\newblock Small-dimensional linear programming and convex hulls made easy.
\newblock {\em Discrete \& Computational Geometry}, 6(3):423--434, 1991.

\bibitem{Seidel93}
R.~Seidel.
\newblock Backwards analysis of randomized geometric algorithms.
\newblock In {\em New Trends in Discrete and Computational Geometry}, pages
  37--67. 1993.

\bibitem{Sen95}
S.~Sen.
\newblock A deterministic $poly(\log\log n)$ time optimal {CRCW PRAM} algorithm
  for linear programming in fixed dimensions.
\newblock Technical report, Department of Computer Science, University of
  Newcastle, 1995.

\bibitem{SBFG}
J.~Shun, G.~E. Blelloch, J.~T. Fineman, P.~B. Gibbons, A.~Kyrola, H.~V.
  Simhadri, and K.~Tangwongsan.
\newblock Brief announcement: the {Problem Based Benchmark Suite}.
\newblock In {\em ACM Symposium on Parallelism in Algorithms and Architectures
  (SPAA)}, pages 68--70, 2012.

\bibitem{SGBFG2015}
J.~Shun, Y.~Gu, G.~Blelloch, J.~Fineman, and P.~Gibbons.
\newblock Sequential random permutation, list contraction and tree contraction
  are highly parallel.
\newblock In {\em ACM-SIAM Symposium on Discrete Algorithms (SODA)}, pages
  431--448, 2015.

\bibitem{slota_ipdps2014_bfs}
G.~M. Slota, S.~Rajamanickam, and K.~Madduri.
\newblock {BFS} and {Coloring-based} parallel algorithms for strongly connected
  components and related problems.
\newblock In {\em International Parallel and Distributed Processing Symposium
  ({IPDPS})}, 2014.

\bibitem{spencer1997time}
T.~H. Spencer.
\newblock Time-work tradeoffs for parallel algorithms.
\newblock {\em Journal of the ACM (JACM)}, 44(5):742--778, 1997.

\bibitem{tarjan1972}
R.~Tarjan.
\newblock Depth-first search and linear graph algorithms.
\newblock {\em SIAM Journal on Computing}, 1(2):146--160, 1972.

\bibitem{Tomkins2015}
D.~Tomkins, T.~Smith, N.~M. Amato, and L.~Rauchwerger.
\newblock Efficient, reachability-based, parallel algorithms for finding
  strongly connected components.
\newblock Technical report, Texas A\&M University, 2015.

\bibitem{ullman1991high}
J.~D. Ullman and M.~Yannakakis.
\newblock High-probability parallel transitive-closure algorithms.
\newblock {\em SIAM Journal on Computing}, 20(1):100--125, 1991.

\bibitem{Vishkin-notes}
U.~Vishkin.
\newblock Thinking in Parallel: Some Basic Data-Parallel Algorithms and Techniques.
\newblock 2010.

\bibitem{Welzl1991}
E.~Welzl.
\newblock Smallest enclosing disks (balls and ellipsoids).
\newblock In {\em New Results and New Trends in Computer Science}, 1991.

\end{thebibliography}


==> trapezoid.tex <==
\section{Planar Trapezoidal Maps}\label{sec:trapezoid}
Planar trapezoidal maps are used to answer the planar point location
problem.  Given a set of non-crossing\footnote{\scriptsize The problem can be
  extended to deal with crossing segments as well.} line segments in
2D as well as a bounding box that contains all of the segments and
defines the region, we can partition the region into trapezoids by
drawing two vertical lines per segment endpoint which extend
vertically above and below the endpoint until hitting the closest
segment (if multiple segments share the same endpoint, then only one
vertical line above and below that endpoint is drawn). We assume that
the set of segments are in general position, meaning that there are no
vertical line segments.  %An example is shown in Figure~\ref{fig:trapezoid}.

%% \begin{figure}
%% \begin{center}  
%%     \includegraphics[width=.8\columnwidth]{figures/trapezoid}
%% \end{center}\vspace{-2em}
%%     \caption{An example of a planar trapezoidal map. }\label{fig:trapezoid}
%% \end{figure} 

The \defn{planar trapezoidal map} problem takes as input a set of
non-crossing line segments as well as a bounding box that contains all
of the segments, and returns a search data structure representing the
trapezoids generated by the segments that can answer the planar point
location query: \emph{Given a point, which trapezoid is it contained
  in?}

The standard sequential randomized incremental algorithm~\cite{BCKO}
begins with an empty bounding box and inserts the segments one-by-one
in a random order. Each insertion generates new trapezoids in the map,
and the search structure is updated accordingly. It has been shown
that a random insertion order leads to an algorithm that takes
$O(n\log n)$ work in expectation, produces a search structure of
$O(n)$ size in expectation, and answers point location queries in
$O(\log n)$ time w.h.p.~\cite{BCKO}.

We define a iteration dependence graph $G_T(S)$ among a set of
segments $S$, where step $j$ depends on step $i < j$ if inserting
segment $j$ deletes any of the trapezoids that segment $i$ generates
in the trapezoidal map. An induction argument shows that this is a
valid dependence graph for the incremental trapezoidal map
algorithm. This algorithm falls into Type 1 of algorithms defined in
Section~\ref{sec:incalg} where the steps have an inverse tail
dependence.

\begin{theorem} \label{theorem:trapezoid}
For $S$ in a random order, for a dependence edge $(i,j)$ in
$G_T(S)$, we have bounded disjoint probability $\hp_i = 8/i$.
\end{theorem}
\begin{proof}
Consider the trapezoidal decomposition at step $i+1$. Each
segment will depend on all the segments above it and below it that can
be reached by traversing a single trapezoid. Thus each segment is a
vertex in the graph, and the trapezoids form edges between
segments. Since this is a planar graph, the average degree of each
vertex is less than 6. Additionally, each segment can interact with at most one
segment to the left and to the right of it. Therefore, on step $i+1$
each segment will depend on fewer than 8 other segments in
expectation. These are picked with equal probability in step $i$, so
$\hp_i = 8/i$. These probabilities are bounded disjoint because two consecutive arcs along a path are not independent. In particular, knowing that
there is an edge between segment $A$ and segment $B$ may make it more
or less likely that the path will be long, depending on the length and
position of segment $B$.
%% Each trapezoid is defined by at most 4 segments, one on the top, one on the
%% bottom, one on the left, and one on the right (there can be multiple
%% segment endpoints on the left side or right side of the trapezoid, but
%% only the first segment that is inserted with an endpoint on that side
%% defines the trapezoid).
%% A backwards analysis shows that during the insertion of the $i+1$'st
%% segment, each trapezoid is removed with probability at most
%% $4/i$~\cite{BCKO}, causing a dependence on the up to 4 segments
%% defining the trapezoid.  Therefore iteration $j$ will depend on at
%% most 16 segments existing at iteration $i < j$, and so $p_{ij} \leq
%% 16/i$.
\end{proof}

Applying Theorems~\ref{thm:lowdepth} and~\ref{theorem:trapezoid} gives
the following corollary.

\begin{corollary} \label{cor:trapezoid}
For $S$ in a random order, the iteration depth of $G_T(S)$ is $O(\log
n)$ w.h.p.
\end{corollary}
%% \begin{proof}
%% We cannot directly apply Theorem~\ref{thm:lowdepth} because two
%% consecutive edges along a path may not be independent. Knowing that
%% there is an edge between segment $A$ and segment $B$ may make it more
%% or less likely that the path will be long, depending on the length and
%% position of segment $B$. However, every other edge along the path will
%% be independent because there is no direct interaction between them. So
%% if we consider all sub-paths consisting of every other edge in the
%% dependence graph, we can apply Theorem~\ref{thm:lowdepth} with
%% $c=16$. The length of the actual path will be twice the length, which
%% does not affect the complexity bound.
%% \end{proof}

The sequential algorithm maintains a search structure throughout the
algorithm that allows point location queries on the current
trapezoidal map. This is also the search structure returned at the end
of the algorithm. The search structure is a DAG, where each leaf is a
trapezoid, and each internal node represents a segment or a point. The
out-degree of each node is constant, and for a random insertion order
the depth of the DAG has been shown to be $O(\log n)$
w.h.p.~\cite{BCKO}.

%% For our parallel algorithm, a segment can identify all of the
%% trapezoids that it affects by doing a breadth-first search (BFS) in
%% the search structure, where only the valid internal nodes and leaves
%% are visited.

To enable efficient parallel construction of the trapezoidal map, we
maintain conflict sets as in~\cite{CS89}, but we have to ensure
that we can perform everything in parallel efficiently. For each
segment, we store in a parallel hash table~\cite{Gil91a} all of the trapezoids in the current
trapezoidal map that the segment is contained in. For each trapezoid,
we store in a parallel hash table all of the unprocessed segments that would remove
the trapezoid if it were inserted, as well as the earliest
(highest-priority) among those segments. If there are multiple
segments sharing an endpoint that affect a trapezoid, we only consider
the earliest segment as a conflict.

Whenever we insert a segment $s$, we take all of the unprocessed
segments in the trapezoids that $s$ is contained in, and assign them
to the new trapezoids that inserting $s$ created.  For each
conflicting segment stored in a trapezoid, we perform $O(1)$ line-side
tests on the at most 4 newly formed trapezoids intersecting this
original trapezoid to determine which trapezoids it now belongs
in. Trapezoids can be assigned multiple copies of the same segment
throughout this process, and inserting into the parallel hash table
will remove duplicates and return the resulting conflict set in
$O(\log n)$ depth w.h.p. and work linear in the size of the conflict sets of
the destroyed trapezoids~\cite{Gil91a}.  Identifying and storing the
earliest conflicting segment per trapezoid can be done with prefix
sums.
%% All of the
%% trapezoids that $s$ affects and the unprocessed segments associated
%% with those trapezoids can be identified, and duplicates removed in
%% $O(\log n)$ depth and work linear in the size of the conflict lists
%% using parallel hashing~\cite{Gil91a}.  
%% Updating the conflict lists of
%% the newly created trapezoids involves taking all of the identified
%% unprocessed segments and performing $O(1)$ line-side tests per segment
%% for each newly created trapezoid.
 %% \julian{I don't think this part is
 %%  work-efficient. The work needs to be proportional to the number of
 %%  unprocessed conflicting segments.}

Updating the conflict sets of these segments involves removing the
deleted trapezoids from the conflict set (we assume we have back
pointers from the trapezoid to the corresponding entry in the conflict
sets of its conflicting segments), then performing a constant number
of line-side tests for the up to 4 newly created trapezoids that
intersect with the destroyed trapezoid, and inserting the trapezoids
that it conflicts with. Again, there can be duplicate trapezoids
inserted, but they will be removed with the hash table.

%% The removal, and line-side tests can all be
%% done in parallel, followed by a pack. Identifying the earliest
%% conflicting segment per trapezoid can be obtained with prefix sums.

The parallel algorithm for trapezoidal maps works in rounds as
follows. Each segment maintains a counter which stores the number of
trapezoids it is the earliest conflicting segment on. The counter can
be computed by having each trapezoid do a fetch-and-add to its
earliest conflicting segment. For any segment whose counter equals the
number of trapezoids it conflicts with, it can proceed to insert
itself and update the trapezoidal map.
%% In each round, all remaining segments in parallel find all of
%% the trapezoids they affect and write their iterate ID to all of the
%% trapezoids that they may affect using a priority-write where a smaller
%% iterate ID has higher priority. Then in parallel, all segments check
%% all of the trapezoids they wrote to, and if all of them contain its
%% ID, it inserts itself into the trapezoidal map, and updates the search
%% structure. 
This guarantees that all of the segments executing in
parallel in a given round will not conflict with each other. The
search structure is updated by deleting the trapezoids destroyed and
adding the newly created trapezoids in a tree, as described
in~\cite{BCKO}. The updates to the search structure can be done in
parallel, as the segments inserted affect disjoint trapezoids, and
hence disjoint portions of the tree. If a segment maintains all of its trapezoids in a finger tree, then it can identify all of its affected trapezoids, and create and delete trapezoids in parallel. 

We first bound the work of the algorithm.  The work of the algorithm
is equal to the sum of the work in (a) maintaining the conflict sets
throughout the algorithm, (b) having trapezoids increment their
earliest segment's counters across all rounds, and (c) updating the
search structure for a segment when it becomes inserted.  The expected
work of (a) in the sequential case has been shown to be $O(n\log
n)$~\cite{CS89}, and since we do everything in parallel
work-efficiently, the work remains $O(n\log n)$.  The work of (b) per
round is $O(n)$ since there are $O(n)$ trapezoids at any time. This
gives a total of $O(n\log n)$ work across all iterations.  Finally,
the expected work of (c) is $O(n\log n)$ as shown
in~\cite{BCKO}. Using the finger trees to identify and update
trapezoids is work-efficient compared to the sequential process of
finding trapezoids by traversing them one-by-one, so the work
complexity is unaffected.


%% To bound (a) we first
%% consider the number of nodes on the search path for any query point
%% $q$. An iteration $i$ contributes a constant number of nodes to the
%% path of $q$ if the trapezoid containing $q$ exists in iteration $i$
%% but not in iteration $i-1$. Each trapezoid can be affected by at most
%% 4 segments, so the probability that this trapezoid is affected by the
%% segment inserted in iteration $i$ is at most $4/i$, giving a path
%% length of at most $\sum_{i=1}^n1/i = O(\log n)$.  Since a segment can
%% be contained in multiple trapezoids, we need to bound the size of the
%% sub-DAG in the search structure that is explored when searching for
%% the segment. Let $k_i$ be the number of trapezoids that segment $i$ is
%% contained in at the beginning of the current round.
%% An upper bound on
%% the number of nodes visited, and hence the overall expected work for
%% searching segment $i$ is $O(k_i\log n)$.
%The expected value of $k_i$ is $O(1)$ by a backwards analysis argument:
%% Inserting segment $i$ causes the creation of $O(k_i)$ trapezoids, so
%% to get a bound on $k_i$ we can compute the expected number of
%% trapezoids created by inserting segment $i$. Using a backwards
%% analysis argument as done in~\cite{BCKO}, removing segment $i$ will
%% cause at most 4 trapezoids to disappear, so inserting $i$ creates each
%% of the $O(i)$ trapezoids with probability at most $4/i$, and $E[k_i] =
%% O(i) \cdot (4/i) = O(1)$.
%% The expected work of (a) per round is
%% $\sum_{i=1}^n{O(E[k_i]\log n)} = O(n\log n)$.
%% Naively multiplying this
%% by the number of rounds gives an expected work of
%% $O(n\log^2n)$.


%% For searching, naively performing the search for all segments per
%% round would give an overall expected work of $O(n\log^2n)$.  Instead
%% of performing the search from scratch each round, each segment only
%% needs to start searching from the sub-DAGs of the trapezoids that it
%% found last time. Therefore, each unprocessed segment $i$ stores $k_i$
%% pointers into the search structure in an array, each pointing to one
%% of the positions of the trapezoids it found in the previous
%% search. Future searches only need to start from these pointers, and we
%% can initialize the BFS with an initial frontier of these $k_i$
%% locations. The overall work performed for searches for segment $i$
%% throughout the algorithm will then be proportional to $O(\log n) +
%% \sum_{j=1}^{O(\log n)}O(E[k_{ji}])$, where $k_{ji}$ is the number of
%% trapezoids segment $i$ is contained in at the beginning of round
%% $j$. Summing over all segments gives an overall expected work of
%% $\sum_{i=1}^n(O(\log n) + \sum_{j=1}^{O(\log n)}O(E[k_{ji}])) =
%% O(n\log n)$ for searching as $E[k_{ji}] = O(1)$ for all $i,j$. The
%% $O(\log n)$ term in the sum comes from the fact that on each round,
%% the depth of the search structure can only increase by $O(1)$, as each
%% newly created trapezoid creates $O(1)$ levels of nodes, and all
%% trapezoids created are in disjoint parts of the search structure.  

%% The
%% work of (b) per round is proportional to the sum of $k_i$'s, which is
%% $O(n)$ in expectation, giving a total of $O(n\log n)$. Finally, the
%% expected work of (c) is $O(n\log n)$ as shown in~\cite{BCKO}.

%% During the search, whenever there is more than one valid choice for
%% the next path to take, we can charge each one of these extra valid
%% choices to a trapezoid that will be found. The first valid choice
%% is charged to the search path of length $O(\log n)$.

%% The visit to each of the trapezoids can be charged to a constant
%% number of internal nodes in the search structure, so the overall
%% work for searching segment $i$ is $O(\log n+k_i)$.


%% A node is created on the search path if in some iteration $i-1$, a
%% trapezoid existed and was destroyed


%%  Each
%% round takes $O(\log n)$ depth for processing the conflict lists, so
%% the depth of the algorithm is $O(\log^2n)$ w.h.p.  The work of the
%% algorithm is equal to the sum of the work in (a) updating the search
%% structure, (b) having iterates write IDs to trapezoids and check what
%% is written, and (c) updating conflict lists.  The overall work of (a)
%% is the same as that of the sequential algorithm~\cite{BCKO}, which is
%% $O(n\log n)$ in expectation.
%% %% The work of (b) is $O(n)$ per round, as a constant number of
%% %% iterates conflict with and will write to a given trapezoid and
%% %% there are $O(n)$ trapezoids.  This contributes $O(n\log n)$ work
%% %% across the $O(\log n)$ rounds.
%% The overall work of (c) is $O(n\log n)$ in expectation, as argued
%% in~\cite{CS89}.

%% Since there are $O(\log
%% n)$ levels of the DAG, the BFS takes at most $O(\log n)$ iterations
%% w.h.p. Each iteration can be implemented in $O(\log^*n)$ depth
%% w.h.p. using approximate compaction~\cite{Gil91a}, for a total of
%% $O(\log n\log^*n)$ depth w.h.p. The overall work is linear in the
%% number of nodes touched.

We now analyze the depth of this algorithm. Each round of the
algorithm processes a level of the dependence graph, and so after
$O(\log n)$ rounds, the algorithm terminates w.h.p. Each round
involves having trapezoids write to counters, inserting segments,
updating the conflict sets, and updating the search
structure. Writing to counters takes $O(1)$ depth with a fetch-and-add
primitive, and can be simulated in $O(\log n)$ depth on a CRCW PRAM
without fetch-and-add~\cite{Matias1990}. Inserting segments and
updating the search structure takes $O(\log n)$ depth for the finger
tree operations.
%% unprocessed segments identifying conflicting trapezoids in
%% the search structure by advancing the BFS by $O(1)$ levels in
%% $O(\log^*n)$ depth w.h.p. using approximate compaction~\cite{Gil91a},
%% and updating the search structure, which can be done in $O(1)$ depth
%% as a segment insertion only affects at most two levels of the search
%% structure. 
Updating the conflict sets takes $O(\log n)$ depth as it
uses packing, prefix sums, and parallel hashing.

%The overall depth is $O(\log n\log^*n)$ w.h.p.

\begin{theorem}
The parallel incremental randomized algorithm for trapezoidal map
construction requires $O(n\log n)$ work in expectation and
$O(\log^2 n)$ depth w.h.p. on an arbitrary-CRCW PRAM.
\end{theorem}

